Colloidal Pivots Enable Brownian Metamaterials and Machines

Biological machines harness targeted deformations that can be actuated by Brownian fluctuations. However, while synthetic micromachines can similarly leverage targeted deformations they are too stiff to be driven by thermal fluctuations and thus require strong forcing. Furthermore, systems that are able to change their conformation by thermal fluctuations do so uncontrollably or require external control. Here we leverage DNA-based sliding contacts to create colloidal pivots, rigid anisotropic objects that freely fluctuate around their pivot point, and use a hierarchical strategy to assemble these into Brownian metamaterials and machines with targeted deformation modes. We realize the archetypical rotating diamond and rotating triangle, or Kagome, geometries, and quantitatively show how thermal fluctuations drive their predicted auxetic deformations. Finally, we implement magnetic particles into the colloidal pivots to achieve an elementary Brownian machine with easily actuatable deformations that can harness Brownian fluctuations. Together, our work introduces a strategy for creating thermal mechanical metamaterials and leverages them for functional Brownian devices, paving the way to materialize flexible, actuatable structures for micro-robots, smart materials, and nano-medicine.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
